Attack on Unfair ToS Clause Detection: A Case Study using Universal Adversarial Triggers

Recent work has demonstrated that natural language processing techniques can support consumer protection by automatically detecting unfair clauses in the Terms of Service (ToS) Agreement. This work demonstrates that transformer-based ToS analysis systems are vulnerable to adversarial attacks. We conduct experiments attacking an unfair-clause detector with universal adversarial triggers. Experiments show that a minor perturbation of the text can considerably reduce the detection performance. Moreover, to measure the detectability of the triggers, we conduct a detailed human evaluation study by collecting both answer accuracy and response time from the participants. The results show that the naturalness of the triggers remains key to tricking readers.

==> figures/len8_performance.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{|l|rrrr|}
\hline
Trigger                                                                                                          & \multicolumn{1}{c}{Length} & \multicolumn{1}{c}{Mode} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c|}{$\Delta$} \\
\hline

Baseline                                                                   & -                          & -                                                  & 80.1                        &                            \\

another witness seems thus admissible scope testify usc                    & 8                          &all                    & 22.6                        & -71.8\%                    \\
assist {[}SEP{]} witness normally justifies cross admissibility willingness & 8                          &no subword                      & 19.2                        & -76.0\%                    \\
% information payment must provide person license rights                     & 7                          & middle                       & lmi                      & 613                        & -23.5\%                   
%   \\
\hline
\end{tabular}
% \vspace{12pt}
\caption{Performance of Universal Triggers on Unfair Label, updated to new results}
% \vspace{-6pt}
\label{tab:len8_trig_perf}
\end{table*}
